Competitive Retrieval: Going Beyond the Single Query

Previous work on the competitive retrieval setting focused on a single-query setting: document authors manipulate their documents so as to improve their future ranking for a given query. We study a competitive setting where authors opt to improve their document's ranking for multiple queries. We use game theoretic analysis to prove that equilibrium does not necessarily exist. We then empirically show that it is more difficult for authors to improve their documents' rankings for multiple queries with a neural ranker than with a state-of-the-art feature-based ranker. We also present an effective approach for predicting the document most highly ranked in the next induced ranking.

==> ack.tex <==
\smallskip
\paragraph*{Acknowledgments}
We thank the reviewers for their helpful comments. This work was supported in part by a Google Faculty Research Award.


==> figures/query_dependent.tex <==
\begin{figure}
\centering
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/query_dependent/querytermscover_improvers}
  \caption{QueryTermsCover}
  \label{fig:querytermscover}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/query_dependent/dir_improvers}
  \caption{LMIR.DIR}
  \label{fig:lmir.dir}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/query_dependent/jm_improvers}
  \caption{LMIR.JM}
  \label{fig:lmir.jm}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/query_dependent/sumtf_improvers}
  \caption{SumTF}
  \label{fig:sumtf}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/query_dependent/sumtfidf_improvers}
  \caption{SumTFIDF}
  \label{fig:sumtfidf}
\end{subfigure}%
\medskip

\caption{Query Dependent Features: Comparison of averaged query dependent feature values for documents that shifted from losing to winning a specific query ($q$) after at least four rounds, categorized by whether their feature values were initially lower/equal to ('\llewq') or higher than ('\lgwq') the eventual winners'. Also depicted are '\wq' for the average query winners' values and '\wt' all the winners in the same topic. The x-axis indicates the negative count of rounds leading up to a win.}
\label{fig:query-dependent}
\end{figure}

==> figures/query_independent.tex <==
\begin{figure}
\centering
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/query_independent/entropy_improvers}
  \caption{Entropy}
  \label{fig:entropy}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/query_independent/stopwordsratio_improvers}
  \caption{StopWordsRatio}
  \label{fig:stopwordsratio}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/query_independent/stopwordscover_improvers}
  \caption{StopWordsCover}
  \label{fig:stopwordscover}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures/query_independent/siminit_improvers}
  \caption{SimInit}
  \label{fig:siminit}
\end{subfigure}%
\medskip

\caption{Query Independent Features: Comparison of averaged query independent feature values for documents that shifted from losing to winning a specific query ($q$) after at least four rounds, categorized by whether their feature values were initially lower/equal to ('\llewq') or higher than ('\lgwq') the eventual winners'. Also depicted are '\wq' for the average query winners' values and '\wt' all the winners in the same topic. The x-axis indicates the negative count of rounds leading up to a win.}
\label{fig:query-independent}
\end{figure}

==> figures2/query_dependent.tex <==
\begin{figure}
\centering
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures2/query_dependent/tf_improvers}
  \caption{TF}
  \label{fig:tf}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures2/query_dependent/normtf_improvers}
  \caption{NormTF}
  \label{fig:normtf}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures2/query_dependent/okapi_improvers}
  \caption{Okapi}
  \label{fig:okapi}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures2/query_dependent/lm_improvers}
  \caption{LM}
  \label{fig:lm}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures2/query_dependent/bert_improvers}
  \caption{BERT}
  \label{fig:bert}
\end{subfigure}%
\medskip

\caption{Averaged query-dependent feature values of documents that lost in at least four consecutive rounds before winning. The documents are grouped based on whether their feature values four rounds before the win were lower than or equal to (\llewq) or higher than (\lgwq) the values of the winners for the given query. \wq and \wt: the averaged feature values of the corresponding winner per query and all the winners per the same topic, respectively. x-axis: the (negative) number of rounds leading up to a win.}
\label{fig:query-dependent}
\end{figure}

==> figures2/query_independent.tex <==
\begin{figure}
\centering
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures2/query_independent/len_improvers}
  \caption{LEN}
  \label{fig:len}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures2/query_independent/fracstop_improvers}
  \caption{FracStop}
  \label{fig:fracstop}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures2/query_independent/stopcover_improvers}
  \caption{StopCover}
  \label{fig:stopcover}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures2/query_independent/ent_improvers}
  \caption{ENT}
  \label{fig:ent}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures2/query_independent/siminit_improvers}
  \caption{SimInit}
  \label{fig:siminit}
\end{subfigure}%
\medskip

\caption{Averaged query-independent feature values of documents that lost in at least four consecutive rounds before winning. The documents are grouped based on whether their feature values four rounds before the win were lower than or equal to (\llewq) or higher than (\lgwq) the values of the winners for the given query. \wq and \wt: the averaged feature values of the corresponding winner per query and all the winners per the same topic, respectively. x-axis: the (negative) number of rounds leading up to a win.}
\label{fig:query-independent}
\end{figure}

==> figures3/query_dependent.tex <==
\begin{figure}
\centering
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures3/query_dependent/tf_improvers}
  \caption{TF}
  \label{fig:tf}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures3/query_dependent/normtf_improvers}
  \caption{NormTF}
  \label{fig:normtf}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures3/query_dependent/okapi_improvers}
  \caption{Okapi}
  \label{fig:okapi}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures3/query_dependent/lm_improvers}
  \caption{LM}
  \label{fig:lm}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures3/query_dependent/bert_improvers}
  \caption{BERT}
  \label{fig:bert}
\end{subfigure}%
\medskip

\caption{Averaged query-dependent feature values of documents that lost in at least four consecutive rounds before winning. The documents are grouped based on whether their feature values four rounds before the win were lower than or equal to (\llewq) or higher than (\lgwq) the values of the winners for the given query. \wq and \wt: the averaged feature values of the corresponding winner per query and all the winners per the same topic, respectively. x-axis: the (negative) number of rounds leading up to a win. Note: in \C and \D, when \bert is used as a standalone ranking function, the feature values of the losing documents are always lower than those of the winning document; therefore, \lgwq is not shown. }
\label{fig:query-dependent}
\end{figure}

==> figures3/query_independent.tex <==
\begin{figure}
\centering
\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures3/query_independent/len_improvers}
  \caption{LEN}
  \label{fig:len}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures3/query_independent/fracstop_improvers}
  \caption{FracStop}
  \label{fig:fracstop}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures3/query_independent/stopcover_improvers}
  \caption{StopCover}
  \label{fig:stopcover}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures3/query_independent/ent_improvers}
  \caption{ENT}
  \label{fig:ent}
\end{subfigure}%
\medskip

\begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=\linewidth]{figures3/query_independent/siminit_improvers}
  \caption{SimInit}
  \label{fig:siminit}
\end{subfigure}%
\medskip

\caption{Averaged query-independent feature values of documents that lost in at least four consecutive rounds before winning. The documents are grouped based on whether their feature values four rounds before the win were lower than or equal to (\llewq) or higher than (\lgwq) the values of the winners for the given query. \wq and \wt: the averaged feature values of the corresponding winner per query and all the winners per the same topic, respectively. x-axis: the (negative) number of rounds leading up to a win.}
\label{fig:query-independent}
\end{figure}

==> sections/dir-ack.tex <==
\smallskip
\noindent
{\bf Acknowledgments}
We thank the reviewers for their comments. This work was supported in part by a Google Faculty Research Award.


==> sections/dir-categories.tex <==
\keywords{ad hoc retrieval; game theory; ranking competition}

%\begin{CCSXML}
%<ccs2012>
%<concept>
%<concept_id>10002951.10003317.10003338.10003340</concept_id>
%<concept_desc>Information systems~Probabilistic retrieval models</concept_desc>
%<concept_significance>300</concept_significance>
%</concept>
%<concept>
%<concept_id>10002951.10003317.10003338.10003341</concept_id>
%<concept_desc>Information systems~Language models</concept_desc>
%<concept_significance>300</concept_significance>
%</concept>
%<concept>
%<concept_id>10002951.10003317.10003338.10003343</concept_id>
%<concept_desc>Information systems~Learning to rank</concept_desc>
%<concept_significance>300</concept_significance>
%</concept>
%</ccs2012>
%\end{CCSXML}

%\ccsdesc[300]{Information systems~Probabilistic retrieval models}
%\ccsdesc[300]{Information systems~Language models}
%\ccsdesc[300]{Information systems~Learning to rank}

\endinput
\vspace*{1mm}
{
\small
\noindent
{\bf Categories and Subject Descriptors:} H.3.3 {[Information Search
and Retrieval]}: {Retrieval models}

\vspace*{1mm}
\noindent
{\bf Keywords:} game theory, ranking competition, strategic publishing
}


==> sections/prompts.tex <==
\subsection{LLM Prompts}
\label{sec:prompts}



%\begin{table*}
%\centering
%\caption{\label{tab:prompts-features} Features of the LLM prompts used by competitors in the competition.}
%\small
%\input{tables/appendix/prompts-features}
%\end{table*}


In the competition, we analyzed the prompts used by competitors in groups \A and \C during rounds 8 to 10.
This analysis aimed to understand the strategies employed by students in generating their documents.
Many students reported not using LLM tools to generate their documents or not modifying their documents in certain rounds.
Despite this, we managed to collect a total of 44 prompts from both groups for our analysis.

% score calculation
An interesting observation is that almost all the students didn't include information about the score calculation in their prompts \footnote{An example of such a prompt: "Since the score is given by the median ranking among 3 queries, we can focus on maximize the rankings on two queries."}.
To be more specific, only three out of 44 prompts mentioned score calculation, with two of these coming from the same student.
Typically, the prompts merely instructed the creation of a document aimed at achieving high rankings for the specified queries.
This indicates that the students likely paid little attention to the mechanism of score calculation, and thus, it did not significantly influence their behavior.
Furthermore, our study aims to explore the dynamics of students competing across multiple queries in a broader sense, rather than concentrating solely on the score calculation mechanism.

% how many prompts even included an example document
The students were provided with an example of a relevant document at the beginning of the competition.
The goal of this example was to provide the students with a reference point for the type of document that would be considered relevant for the queries.
Out of the 44 prompts, 29 prompts included some example document—whether it was the original example document, the student's own document from the last round, or the document of another student from the same group.
This promotes originality and diversity in the documents submitted by the students in the competition.
%\haya{How can we measure originality? diversity?}
Moreover, this indicates that the students were likely influenced by the example document when generating their own documents.

% how many prompts included the winning document
24 prompts included at least one of the winning documents from the previous round, but only 5 prompts included all documents from the previous round.
Moreover, just 3 prompts included their own document from the previous round, and did not include the winning documents.
This suggests that the students considered the winning documents as the most effective examples to learn from and to use as a foundation for their own documents.


% none of the prompts included history before last round (markovian)
As described in Section~\ref{sec:bots}, the bots we used differed in their ability to remember the history of the competition ("memory level").
In particular, the \markov bot was able to remember the history of the competition up to the previous round, while the \nonmarkov bot was able to remember the entire history of the competition.
However, none of the prompts created by students included any information about the history of the competition before the last round.
In terms of agents, this means that the students behaved like \markov bots.




%In order to systematically analyze the prompts used by the competitors, we identified 15 binary features, each representing a distinct aspect of the prompt content.
%Table~\ref{tab:prompts-features} summarizes these features along with the number of times each feature was positively identified in the prompts.
%
%
%For each of the binary features, the average rank, median rank, raw promotion and scaled promotion (last two w.r.t. median rank) were compared between the following groups:
%
%\begin{itemize}
%    \item \textbf{with strategy}: students that reported their prompts and their feature value is \textit{true}.
%    \item \textbf{without strategy}: students that reported their prompts and their feature value is \textit{false}.
%    \item \textbf{students}: all students for which the feature value is not \textit{true} (either \textit{false} or didn't report their prompt).
%    \item \textbf{dummy}: static bot with initial document.
%\end{itemize}
%
%Each feature is represented by its own table.
%Within these tables, the cell values denote the average values for their respective groups.
%Cells are colored in blue if the results are better than the results of the 'with strategy' group, and red otherwise.
%If the difference from the 'with strategy' group are significant, the cell is underlined.
%Significance was assessed using an independent two-sample t-test with a significance level set at 0.05.
%Note that for "average rank" and "median rank" a lower value is preferable, and the opposite for "raw promotion" and "scaled promotion".
%
%%\input{tables/appendix/competition-background-(score-calculation)}
%%
%%In general,

==> tables-simple/analysis/num_wins.tex <==
\begin{tabular}{llll}
\toprule
Number of Wins & 1 & 2 & 3 \\
\midrule
\A & 17.86\% & 17.03\% & 65.11\% \\
\B & 17.73\% & 15.24\% & 67.04\% \\
\C & 62.94\% & 28.48\% & 8.58\% \\
\D & 65.67\% & 27.59\% & 6.74\% \\
\bottomrule
\end{tabular}


==> tables-simple/data/groups-description.tex <==
\begin{tabular}{|c|c|c|}
    \hline
    \textbf{Group} & \textbf{Ranking Function} & \textbf{LM Tools} \\
    \hline
    A & LambdaMART & Allowed \\
    \hline
    B & LambdaMART & Prohibited \\
    \hline
    C & BERT & Allowed \\
    \hline
    D & BERT & Prohibited \\
    \hline
\end{tabular}

==> tables-simple/prediction/ablation.tex <==
\subcaption*{\A}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{LReg} & \multicolumn{2}{c}{LSVM} & \multicolumn{2}{c}{PSVM} & \multicolumn{2}{c}{RForest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
  &  &  &  &  &  &  &  &  \\
\midrule
\metaFt + \atomicFt & 0.714 & 0.698 & 0.711 & 0.694 & 0.746 & 0.728 & 0.757 & 0.743 \\
\docLen + \metaFt + \atomicFt & 0.835 & 0.824 & 0.829 & 0.817 & 0.882 & 0.872 & 0.896 & 0.889 \\
\centroidMacro + \metaFt + \atomicFt & 0.79 & 0.775 & 0.794 & 0.779 & 0.788 & 0.772 & 0.821 & 0.808 \\
\metaFt + \atomicFt + \QueryPrev & 0.746 & 0.731 & 0.744 & 0.729 & 0.763 & 0.746 & 0.779 & 0.764 \\
\metaFt + \atomicFt + \PrevPosition & 0.752 & 0.736 & 0.745 & 0.729 & 0.831 & 0.819 & 0.835 & 0.823 \\
\metaFt + \atomicFt + \PrevImprove & 0.686 & 0.671 & 0.666 & 0.649 & 0.769 & 0.756 & 0.753 & 0.74 \\
\centroidMacro + \docLen + \metaFt + \atomicFt + \PrevPosition + \QueryPrev + \PrevImprove & 0.858 & 0.847 & 0.87 & 0.858 & 0.891 & 0.881 & 0.843 & 0.832 \\
\docLen + \metaFt + \QueryPrev & \textbf{0.912} & \textbf{0.905} & \textbf{0.912} & \textbf{0.905} & 0.874 & 0.863 & 0.873 & 0.864 \\
\bottomrule
\end{tabular}

\bigskip
\subcaption*{\B}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{LReg} & \multicolumn{2}{c}{LSVM} & \multicolumn{2}{c}{PSVM} & \multicolumn{2}{c}{RForest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
  &  &  &  &  &  &  &  &  \\
\midrule
\metaFt + \atomicFt & 0.721 & 0.708 & 0.708 & 0.694 & 0.699 & 0.685 & 0.791 & 0.783 \\
\docLen + \metaFt + \atomicFt & 0.866 & 0.858 & 0.868 & 0.861 & 0.823 & 0.813 & 0.878 & 0.871 \\
\centroidMacro + \metaFt + \atomicFt & 0.738 & 0.727 & 0.733 & 0.721 & 0.722 & 0.708 & 0.785 & 0.777 \\
\metaFt + \atomicFt + \QueryPrev & 0.747 & 0.735 & 0.743 & 0.731 & 0.711 & 0.699 & 0.801 & 0.793 \\
\metaFt + \atomicFt + \PrevPosition & 0.694 & 0.68 & 0.683 & 0.669 & 0.73 & 0.719 & 0.765 & 0.756 \\
\metaFt + \atomicFt + \PrevImprove & 0.756 & 0.74 & 0.763 & 0.749 & 0.696 & 0.682 & 0.792 & 0.782 \\
\centroidMacro + \docLen + \metaFt + \atomicFt + \PrevPosition + \QueryPrev + \PrevImprove & 0.838 & 0.83 & 0.865 & 0.858 & 0.865 & 0.859 & 0.847 & 0.838 \\
\docLen + \atomicFt + \PrevPosition + \QueryPrev + \PrevImprove & 0.909 & 0.903 & \textbf{0.914} & \textbf{0.908} & 0.838 & 0.828 & 0.862 & 0.852 \\
\bottomrule
\end{tabular}

\bigskip
\subcaption*{\C}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{LReg} & \multicolumn{2}{c}{LSVM} & \multicolumn{2}{c}{PSVM} & \multicolumn{2}{c}{RForest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
  &  &  &  &  &  &  &  &  \\
\midrule
\metaFt + \atomicFt & 0.722 & 0.701 & 0.715 & 0.694 & 0.669 & 0.645 & 0.713 & 0.692 \\
\docLen + \metaFt + \atomicFt & 0.709 & 0.687 & 0.702 & 0.679 & 0.659 & 0.633 & 0.712 & 0.69 \\
\centroidMacro + \metaFt + \atomicFt & 0.71 & 0.688 & 0.702 & 0.68 & 0.653 & 0.627 & 0.703 & 0.68 \\
\metaFt + \atomicFt + \QueryPrev & 0.728 & 0.707 & 0.725 & 0.704 & 0.697 & 0.672 & 0.709 & 0.687 \\
\metaFt + \atomicFt + \PrevPosition & 0.772 & 0.755 & 0.771 & 0.754 & 0.767 & 0.749 & 0.761 & 0.744 \\
\metaFt + \atomicFt + \PrevImprove & 0.73 & 0.713 & 0.746 & 0.729 & 0.712 & 0.692 & 0.771 & 0.755 \\
\centroidMacro + \docLen + \metaFt + \atomicFt + \PrevPosition + \QueryPrev + \PrevImprove & 0.811 & 0.797 & 0.803 & 0.788 & 0.814 & 0.798 & 0.826 & 0.812 \\
\metaFt + \atomicFt + \PrevPosition + \QueryPrev + \PrevImprove & 0.814 & 0.8 & 0.814 & 0.8 & 0.824 & 0.81 & \textbf{0.838} & \textbf{0.825} \\
\bottomrule
\end{tabular}

\bigskip
\subcaption*{\D}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{LReg} & \multicolumn{2}{c}{LSVM} & \multicolumn{2}{c}{PSVM} & \multicolumn{2}{c}{RForest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
  &  &  &  &  &  &  &  &  \\
\midrule
\metaFt + \atomicFt & 0.733 & 0.727 & 0.742 & 0.735 & 0.642 & 0.635 & 0.72 & 0.712 \\
\docLen + \metaFt + \atomicFt & 0.754 & 0.748 & 0.76 & 0.753 & 0.637 & 0.629 & 0.718 & 0.71 \\
\centroidMacro + \metaFt + \atomicFt & 0.752 & 0.745 & 0.762 & 0.755 & 0.656 & 0.648 & 0.712 & 0.704 \\
\metaFt + \atomicFt + \QueryPrev & 0.717 & 0.71 & 0.726 & 0.719 & 0.655 & 0.647 & 0.734 & 0.727 \\
\metaFt + \atomicFt + \PrevPosition & 0.725 & 0.716 & 0.721 & 0.713 & 0.748 & 0.741 & 0.747 & 0.739 \\
\metaFt + \atomicFt + \PrevImprove & 0.717 & 0.712 & 0.715 & 0.709 & 0.661 & 0.655 & 0.73 & 0.725 \\
\centroidMacro + \docLen + \metaFt + \atomicFt + \PrevPosition + \QueryPrev + \PrevImprove & 0.781 & 0.774 & 0.784 & 0.778 & 0.785 & 0.779 & 0.752 & 0.746 \\
\centroidMacro + \metaFt + \atomicFt + \PrevPosition + \PrevImprove & 0.809 & 0.803 & \textbf{0.819} & \textbf{0.814} & 0.701 & 0.696 & 0.751 & 0.744 \\
\bottomrule
\end{tabular}



==> tables-simple/prediction/baselines_results.tex <==
\begin{tabular}{llrrrrrrrr}
  \toprule
 &  & \random & \majority & \awinner & \aloser & \lreg & \lsvm & \psvm & \rforest \\
 &  &  &  &  &  &  &  &  &  \\
 \midrule
\A & \acc & 0.647 & 0.395 & 0.466 & 0.534 & 0.714 & 0.711 & 0.746 & 0.757 \\
\A & \FOne & 0.622 & 0.351 & 0.636 & 0.0 & 0.698 & 0.694 & 0.728 & 0.743 \\
  \midrule
\B & \acc & 0.758 & 0.406 & 0.476 & 0.524 & 0.721 & 0.708 & 0.699 & 0.791 \\
\B & \FOne & 0.745 & 0.376 & 0.645 & 0.0 & 0.708 & 0.694 & 0.685 & 0.783 \\
  \midrule
\C & \acc & 0.689 & 0.509 & 0.464 & 0.536 & 0.722 & 0.715 & 0.669 & 0.713 \\
\C & \FOne & 0.664 & 0.47 & 0.634 & 0.0 & 0.701 & 0.694 & 0.645 & 0.692 \\
  \midrule
\D & \acc & 0.648 & 0.461 & 0.487 & 0.513 & 0.733 & 0.742 & 0.642 & 0.72 \\
\D & \FOne & 0.638 & 0.446 & 0.655 & 0.0 & 0.727 & 0.735 & 0.635 & 0.712 \\
 \bottomrule
\end{tabular}


==> tables/analysis/num_wins.tex <==
\begin{tabular}{llll}
\toprule
Number of Wins & 1 & 2 & 3 \\
\midrule
\A & 17.86\% & 17.03\% & 65.11\% \\
\B & 17.73\% & 15.24\% & 67.04\% \\
\C & 62.94\% & 28.48\% & 8.58\% \\
\D & 65.67\% & 27.59\% & 6.74\% \\
\bottomrule
\end{tabular}


==> tables/analysis/num_wins_in_match_worst_rank_all.tex <==
\begin{tabular}{lllllllll}
\toprule
 & \multicolumn{2}{c}{\A} & \multicolumn{2}{c}{\B} & \multicolumn{2}{c}{\C} & \multicolumn{2}{c}{\D} \\
 & \docsPercentage & \avgRank & \docsPercentage & \avgRank & \docsPercentage & \avgRank & \docsPercentage & \avgRank \\
\midrule
\OneWin & 17.9\% & 2.3 & 17.7\% & 2.6 & 62.9\% & 3.8 & 65.7\% & 4.0 \\
\TwoWins & 17.0\% & 2.1 & 15.2\% & 2.3 & 28.5\% & 3.3 & 27.6\% & 3.2 \\
\ThreeWins & 65.1\% & - & 67.0\% & - & 8.6\% & - & 6.7\% & - \\
\bottomrule
\end{tabular}


==> tables/analysis/num_wins_transposed.tex <==
\begin{tabular}{lllll}
\toprule
 & \A & \B & \C & \D \\
\midrule
\OneWin & 17.86\% & 17.73\% & 62.94\% & 65.67\% \\
\TwoWins & 17.03\% & 15.24\% & 28.48\% & 27.59\% \\
\ThreeWins & 65.11\% & 67.04\% & 8.58\% & 6.74\% \\
\bottomrule
\end{tabular}


==> tables/analysis/rank_by_num_wins.tex <==
\begin{tabular}{lrrrr}
\toprule
 & \A & \B & \C & \D \\
\midrule
\OneWin & 2.184615 & 2.429688 & 3.356041 & 3.465394 \\
\TwoWins & 2.112903 & 2.290909 & 3.255682 & 3.187500 \\
\bottomrule
\end{tabular}


==> tables/prediction/ablation_remove.tex <==
\subcaption*{$LTR \wedge LLM$}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{LReg} & \multicolumn{2}{c}{LSVM} & \multicolumn{2}{c}{PSVM} & \multicolumn{2}{c}{RForest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
  &  &  &  &  &  &  &  &  \\
\midrule
$\neg$ \atomicFt & \textbf{0.878} & \textbf{0.87} & \textbf{0.881} & \textbf{0.873} & \textbf{0.897} & \textbf{0.888} & 0.878 & 0.87 \\
$\neg$ \docLen & 0.786 & 0.771 & 0.761 & 0.745 & 0.838 & 0.825 & 0.806 & 0.792 \\
$\neg$ \centroidMacro & 0.848 & 0.835 & 0.847 & 0.833 & 0.852 & 0.839 & 0.839 & 0.828 \\
$\neg$ \QueryPrev & 0.866 & 0.857 & 0.869 & 0.859 & 0.884 & 0.873 & 0.837 & 0.827 \\
$\neg$ \metaFt & 0.851 & 0.838 & 0.86 & 0.847 & 0.864 & 0.853 & 0.838 & 0.826 \\
$\neg$ \PrevPosition & 0.846 & 0.834 & 0.868 & 0.857 & 0.884 & 0.875 & 0.854 & 0.842 \\
$\neg$ \PrevImprove & 0.831 & 0.82 & 0.829 & 0.818 & 0.876 & 0.866 & \textbf{0.885} & \textbf{0.876} \\
\centroidMacro + \docLen + \metaFt + \atomicFt + \PrevPosition + \QueryPrev + \PrevImprove & 0.858 & 0.847 & 0.87 & 0.858 & 0.891 & 0.881 & 0.843 & 0.832 \\
\bottomrule
\end{tabular}

\bigskip
\subcaption*{$LTR \wedge \neg LLM$}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{LReg} & \multicolumn{2}{c}{LSVM} & \multicolumn{2}{c}{PSVM} & \multicolumn{2}{c}{RForest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
  &  &  &  &  &  &  &  &  \\
\midrule
$\neg$ \atomicFt & 0.819 & 0.807 & 0.81 & 0.798 & 0.82 & 0.811 & 0.834 & 0.824 \\
$\neg$ \docLen & 0.739 & 0.723 & 0.74 & 0.724 & 0.76 & 0.748 & 0.795 & 0.785 \\
$\neg$ \centroidMacro & 0.841 & 0.833 & 0.862 & 0.855 & 0.848 & 0.841 & 0.846 & 0.837 \\
$\neg$ \QueryPrev & 0.829 & 0.821 & 0.842 & 0.835 & 0.823 & 0.817 & 0.835 & 0.827 \\
$\neg$ \metaFt & \textbf{0.897} & \textbf{0.89} & \textbf{0.91} & \textbf{0.903} & 0.84 & 0.831 & 0.855 & 0.844 \\
$\neg$ \PrevPosition & 0.869 & 0.862 & 0.868 & 0.861 & 0.762 & 0.752 & \textbf{0.867} & \textbf{0.86} \\
$\neg$ \PrevImprove & 0.884 & 0.877 & 0.881 & 0.875 & \textbf{0.867} & \textbf{0.86} & 0.86 & 0.853 \\
\centroidMacro + \docLen + \metaFt + \atomicFt + \PrevPosition + \QueryPrev + \PrevImprove & 0.838 & 0.83 & 0.865 & 0.858 & 0.865 & 0.859 & 0.847 & 0.838 \\
\bottomrule
\end{tabular}

\bigskip
\subcaption*{$SEM \wedge LLM$}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{LReg} & \multicolumn{2}{c}{LSVM} & \multicolumn{2}{c}{PSVM} & \multicolumn{2}{c}{RForest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
  &  &  &  &  &  &  &  &  \\
\midrule
$\neg$ \atomicFt & 0.775 & 0.76 & 0.772 & 0.757 & 0.777 & 0.76 & 0.773 & 0.756 \\
$\neg$ \docLen & 0.814 & 0.8 & \textbf{0.814} & \textbf{0.8} & \textbf{0.815} & \textbf{0.799} & \textbf{0.837} & \textbf{0.824} \\
$\neg$ \centroidMacro & 0.812 & 0.798 & 0.799 & 0.783 & 0.813 & 0.798 & 0.823 & 0.81 \\
$\neg$ \QueryPrev & \textbf{0.821} & \textbf{0.807} & 0.779 & 0.764 & 0.763 & 0.744 & 0.802 & 0.787 \\
$\neg$ \metaFt & 0.755 & 0.738 & 0.76 & 0.743 & 0.741 & 0.72 & 0.802 & 0.786 \\
$\neg$ \PrevPosition & 0.756 & 0.739 & 0.766 & 0.749 & 0.733 & 0.713 & 0.784 & 0.768 \\
$\neg$ \PrevImprove & 0.755 & 0.736 & 0.759 & 0.74 & 0.746 & 0.727 & 0.781 & 0.765 \\
\centroidMacro + \docLen + \metaFt + \atomicFt + \PrevPosition + \QueryPrev + \PrevImprove & 0.811 & 0.797 & 0.803 & 0.788 & 0.814 & 0.798 & 0.826 & 0.812 \\
\bottomrule
\end{tabular}

\bigskip
\subcaption*{$SEM \wedge \neg LLM$}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{LReg} & \multicolumn{2}{c}{LSVM} & \multicolumn{2}{c}{PSVM} & \multicolumn{2}{c}{RForest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
  &  &  &  &  &  &  &  &  \\
\midrule
$\neg$ \atomicFt & 0.713 & 0.706 & 0.718 & 0.712 & 0.751 & 0.746 & 0.716 & 0.709 \\
$\neg$ \docLen & 0.772 & 0.765 & 0.769 & 0.762 & 0.771 & 0.765 & 0.755 & 0.748 \\
$\neg$ \centroidMacro & 0.694 & 0.688 & 0.68 & 0.673 & 0.72 & 0.714 & \textbf{0.759} & \textbf{0.753} \\
$\neg$ \QueryPrev & \textbf{0.784} & \textbf{0.779} & \textbf{0.807} & \textbf{0.802} & 0.682 & 0.676 & 0.749 & 0.742 \\
$\neg$ \metaFt & 0.703 & 0.696 & 0.699 & 0.691 & 0.752 & 0.746 & 0.728 & 0.721 \\
$\neg$ \PrevPosition & 0.772 & 0.766 & 0.771 & 0.766 & 0.765 & 0.759 & 0.734 & 0.728 \\
$\neg$ \PrevImprove & 0.761 & 0.754 & 0.772 & 0.765 & 0.731 & 0.723 & 0.739 & 0.73 \\
\centroidMacro + \docLen + \metaFt + \atomicFt + \PrevPosition + \QueryPrev + \PrevImprove & 0.781 & 0.774 & 0.784 & 0.778 & \textbf{0.785} & \textbf{0.779} & 0.752 & 0.746 \\
\bottomrule
\end{tabular}



==> tables/prediction/ablation_remove_LReg.tex <==
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{\A} & \multicolumn{2}{c}{\B} & \multicolumn{2}{c}{\C} & \multicolumn{2}{c}{\D} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
\midrule
$\neg$ \atomicFt & $\mathbf{0.874}$ & $\mathbf{0.867}$ & $0.829^*$ & $0.818^*$ & $0.766$ & $0.749$ & $0.694$ & $0.687$ \\
$\neg$ \metaFt & $0.812$ & $0.798$ & $0.902$ & $0.897$ & $0.734^*$ & $0.713^*$ & $0.667^*$ & $0.658^*$ \\
$\neg$ \centroidMacro & $0.864$ & $0.853$ & $0.886$ & $0.879$ & $\mathbf{0.815}$ & $\mathbf{0.801}$ & $0.639^*$ & $0.630^*$ \\
$\neg$ \docLen & $0.812$ & $0.800$ & $0.756^*$ & $0.743^*$ & $0.798$ & $0.783$ & $\mathbf{0.759}$ & $0.752$ \\
$\neg$ \PrevPosition & $0.864$ & $0.855$ & $0.870$ & $0.864$ & $0.766$ & $0.748$ & $0.713$ & $0.707$ \\
$\neg$ \QueryPrev & $0.832$ & $0.823$ & $0.837^*$ & $0.830^*$ & $\mathbf{0.815}$ & $0.800$ & $\mathbf{0.759}$ & $\mathbf{0.753}$ \\
$\neg$ \PrevImprove & $0.759$ & $0.741$ & $\mathbf{0.919}^*$ & $\mathbf{0.914}^*$ & $\mathbf{0.815}$ & $0.800$ & $0.741$ & $0.734$ \\
\allPredFeatures & $0.822$ & $0.810$ & $0.886$ & $0.879$ & $\mathbf{0.815}$ & $0.800$ & $0.750$ & $0.742$ \\
\bottomrule
\end{tabular}


==> tables/prediction/ablation_remove_LSVM.tex <==
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{\A} & \multicolumn{2}{c}{\B} & \multicolumn{2}{c}{\C} & \multicolumn{2}{c}{\D} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
\midrule
$\neg$ \atomicFt & $\mathbf{0.885}$ & $\mathbf{0.878}$ & $0.829$ & $0.818$ & $0.766$ & $0.748$ & $0.694$ & $0.686$ \\
$\neg$ \metaFt & $0.832$ & $0.819$ & $\mathbf{0.902}$ & $0.897$ & $0.766$ & $0.748$ & $0.657^*$ & $0.649^*$ \\
$\neg$ \centroidMacro & $0.822$ & $0.807$ & $0.878$ & $0.871$ & $0.806$ & $0.791$ & $0.630^*$ & $0.621^*$ \\
$\neg$ \docLen & $0.770^*$ & $0.756^*$ & $0.732^*$ & $0.717^*$ & $0.782$ & $0.765$ & $0.741$ & $0.733$ \\
$\neg$ \PrevPosition & $\mathbf{0.885}$ & $0.876$ & $0.878$ & $0.872$ & $0.766$ & $0.747$ & $0.722$ & $0.716$ \\
$\neg$ \QueryPrev & $0.843$ & $0.831$ & $0.854$ & $0.846$ & $0.790$ & $0.774$ & $\mathbf{0.787}$ & $\mathbf{0.780}$ \\
$\neg$ \PrevImprove & $0.864$ & $0.854$ & $\mathbf{0.902}$ & $\mathbf{0.898}$ & $\mathbf{0.831}$ & $\mathbf{0.817}$ & $0.769$ & $0.762$ \\
\allPredFeatures & $0.853$ & $0.843$ & $0.870$ & $0.863$ & $0.798$ & $0.782$ & $0.750$ & $0.742$ \\
\bottomrule
\end{tabular}


==> tables/prediction/ablation_remove_PSVM.tex <==
\begin{tabular}{@{}lllllllll@{}}
\toprule
  & \multicolumn{2}{c}{\A} & \multicolumn{2}{c}{\B} & \multicolumn{2}{c}{\C} & \multicolumn{2}{c}{\D} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
\midrule
\atomicFt & $\mathbf{0.895}$ & $\mathbf{0.887}$ & $0.821$ & $0.814$ & $0.782$ & $0.764$ & $0.722^*$ & $0.716^*$ \\
\metaFt & $0.874$ & $0.862$ & $\mathbf{0.878}$ & $\mathbf{0.872}$ & $0.790$ & $0.772$ & $0.731$ & $0.725$ \\
\centroidMacro & $0.822$ & $0.809$ & $0.846$ & $0.837$ & $0.831$ & $0.816$ & $0.676^*$ & $0.668^*$ \\
\docLen & $0.812^*$ & $0.798^*$ & $0.756^*$ & $0.746^*$ & $0.815$ & $0.799$ & $\mathbf{0.796}$ & $\mathbf{0.792}$ \\
\PrevPosition & $\mathbf{0.895}$ & $\mathbf{0.887}$ & $0.862$ & $0.855$ & $0.710^*$ & $0.686^*$ & $0.750$ & $0.744$ \\
\QueryPrev & $0.864$ & $0.851$ & $0.764^*$ & $0.757^*$ & $0.782$ & $0.765$ & $0.657^*$ & $0.649^*$ \\
\PrevImprove & $0.812^*$ & $0.800^*$ & $0.870$ & $0.863$ & $\mathbf{0.839}$ & $\mathbf{0.826}$ & $0.769$ & $0.764$ \\ \midrule
\allPredFeatures & $\mathbf{0.895}$ & $0.885$ & $0.846$ & $0.839$ & $0.806$ & $0.790$ & $\mathbf{0.796}$ & $0.790$ \\
\bottomrule
\end{tabular}


==> tables/prediction/ablation_remove_RForest.tex <==
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{\A} & \multicolumn{2}{c}{\B} & \multicolumn{2}{c}{\C} & \multicolumn{2}{c}{\D} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
\midrule
$\neg$ \atomicFt & $\mathbf{0.843}$ & $\mathbf{0.834}$ & $0.797$ & $0.786$ & $0.806$ & $0.790$ & $0.722$ & $0.715$ \\
$\neg$ \metaFt & $\mathbf{0.843}$ & $0.831$ & $\mathbf{0.846}$ & $\mathbf{0.835}$ & $0.831$ & $0.818$ & $0.685$ & $0.678$ \\
$\neg$ \centroidMacro & $0.822$ & $0.812$ & $0.813$ & $0.804$ & $0.823$ & $0.808$ & $0.694$ & $0.687$ \\
$\neg$ \docLen & $0.812$ & $0.796$ & $0.748^*$ & $0.737^*$ & $\mathbf{0.863}$ & $0.851$ & $0.713$ & $0.704$ \\
$\neg$ \PrevPosition & $\mathbf{0.843}$ & $0.830$ & $0.837$ & $0.828$ & $0.806^*$ & $0.790^*$ & $0.694$ & $0.687$ \\
$\neg$ \QueryPrev & $0.791^*$ & $0.774$ & $0.805$ & $0.795$ & $0.798^*$ & $0.781^*$ & $\mathbf{0.750}$ & $\mathbf{0.743}$ \\
$\neg$ \PrevImprove & $0.791^*$ & $0.775^*$ & $0.813$ & $0.804$ & $\mathbf{0.863}$ & $\mathbf{0.852}$ & $0.731$ & $0.724$ \\
\allPredFeatures & $\mathbf{0.843}$ & $0.832$ & $0.837$ & $0.831$ & $0.855$ & $0.842$ & $\mathbf{0.750}$ & $\mathbf{0.743}$ \\
\bottomrule
\end{tabular}


==> tables/prediction/ablation_remove_all.tex <==
\subcaption*{\A}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{\lreg} & \multicolumn{2}{c}{\lsvm} & \multicolumn{2}{c}{\psvm} & \multicolumn{2}{c}{\rforest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
\midrule
$\neg$ \atomicFt & $\mathbf{0.874}$ & $\mathbf{0.867}$ & $\mathbf{0.885}$ & $\mathbf{0.878}$ & $\mathbf{0.895}$ & $\mathbf{0.887}$ & $\mathbf{0.843}$ & $\mathbf{0.834}$ \\
$\neg$ \metaFt & $0.812$ & $0.798$ & $0.832$ & $0.819$ & $0.874$ & $0.862$ & $\mathbf{0.843}$ & $0.831$ \\
$\neg$ \centroidMacro & $0.864$ & $0.853$ & $0.822$ & $0.807$ & $0.822$ & $0.809$ & $0.822$ & $0.812$ \\
$\neg$ \docLen & $0.812$ & $0.800$ & $0.770^*$ & $0.756^*$ & $0.812^*$ & $0.798^*$ & $0.812$ & $0.796$ \\
$\neg$ \PrevPosition & $0.864$ & $0.855$ & $\mathbf{0.885}$ & $0.876$ & $\mathbf{0.895}$ & $\mathbf{0.887}$ & $\mathbf{0.843}$ & $0.830$ \\
$\neg$ \QueryPrev & $0.832$ & $0.823$ & $0.843$ & $0.831$ & $0.864$ & $0.851$ & $0.791^*$ & $0.774$ \\
$\neg$ \PrevImprove & $0.759$ & $0.741$ & $0.864$ & $0.854$ & $0.812^*$ & $0.800^*$ & $0.791^*$ & $0.775^*$ \\
\allPredFeatures & $0.822$ & $0.810$ & $0.853$ & $0.843$ & $\mathbf{0.895}$ & $0.885$ & $\mathbf{0.843}$ & $0.832$ \\
\bottomrule
\end{tabular}

\bigskip
\subcaption*{\B}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{\lreg} & \multicolumn{2}{c}{\lsvm} & \multicolumn{2}{c}{\psvm} & \multicolumn{2}{c}{\rforest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
\midrule
$\neg$ \atomicFt & $0.829^*$ & $0.818^*$ & $0.829$ & $0.818$ & $0.821$ & $0.814$ & $0.797$ & $0.786$ \\
$\neg$ \metaFt & $0.902$ & $0.897$ & $\mathbf{0.902}$ & $0.897$ & $\mathbf{0.878}$ & $\mathbf{0.872}$ & $\mathbf{0.846}$ & $\mathbf{0.835}$ \\
$\neg$ \centroidMacro & $0.886$ & $0.879$ & $0.878$ & $0.871$ & $0.846$ & $0.837$ & $0.813$ & $0.804$ \\
$\neg$ \docLen & $0.756^*$ & $0.743^*$ & $0.732^*$ & $0.717^*$ & $0.756^*$ & $0.746^*$ & $0.748^*$ & $0.737^*$ \\
$\neg$ \PrevPosition & $0.870$ & $0.864$ & $0.878$ & $0.872$ & $0.862$ & $0.855$ & $0.837$ & $0.828$ \\
$\neg$ \QueryPrev & $0.837^*$ & $0.830^*$ & $0.854$ & $0.846$ & $0.764^*$ & $0.757^*$ & $0.805$ & $0.795$ \\
$\neg$ \PrevImprove & $\mathbf{0.919}^*$ & $\mathbf{0.914}^*$ & $\mathbf{0.902}$ & $\mathbf{0.898}$ & $0.870$ & $0.863$ & $0.813$ & $0.804$ \\
\allPredFeatures & $0.886$ & $0.879$ & $0.870$ & $0.863$ & $0.846$ & $0.839$ & $0.837$ & $0.831$ \\
\bottomrule
\end{tabular}

\bigskip
\subcaption*{\C}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{\lreg} & \multicolumn{2}{c}{\lsvm} & \multicolumn{2}{c}{\psvm} & \multicolumn{2}{c}{\rforest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
\midrule
$\neg$ \atomicFt & $0.766$ & $0.749$ & $0.766$ & $0.748$ & $0.782$ & $0.764$ & $0.806$ & $0.790$ \\
$\neg$ \metaFt & $0.734^*$ & $0.713^*$ & $0.766$ & $0.748$ & $0.790$ & $0.772$ & $0.831$ & $0.818$ \\
$\neg$ \centroidMacro & $\mathbf{0.815}$ & $\mathbf{0.801}$ & $0.806$ & $0.791$ & $0.831$ & $0.816$ & $0.823$ & $0.808$ \\
$\neg$ \docLen & $0.798$ & $0.783$ & $0.782$ & $0.765$ & $0.815$ & $0.799$ & $\mathbf{0.863}$ & $0.851$ \\
$\neg$ \PrevPosition & $0.766$ & $0.748$ & $0.766$ & $0.747$ & $0.710^*$ & $0.686^*$ & $0.806^*$ & $0.790^*$ \\
$\neg$ \QueryPrev & $\mathbf{0.815}$ & $0.800$ & $0.790$ & $0.774$ & $0.782$ & $0.765$ & $0.798^*$ & $0.781^*$ \\
$\neg$ \PrevImprove & $\mathbf{0.815}$ & $0.800$ & $\mathbf{0.831}$ & $\mathbf{0.817}$ & $\mathbf{0.839}$ & $\mathbf{0.826}$ & $\mathbf{0.863}$ & $\mathbf{0.852}$ \\
\allPredFeatures & $\mathbf{0.815}$ & $0.800$ & $0.798$ & $0.782$ & $0.806$ & $0.790$ & $0.855$ & $0.842$ \\
\bottomrule
\end{tabular}

\bigskip
\subcaption*{\D}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{\lreg} & \multicolumn{2}{c}{\lsvm} & \multicolumn{2}{c}{\psvm} & \multicolumn{2}{c}{\rforest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
\midrule
$\neg$ \atomicFt & $0.694$ & $0.687$ & $0.694$ & $0.686$ & $0.722^*$ & $0.716^*$ & $0.722$ & $0.715$ \\
$\neg$ \metaFt & $0.667^*$ & $0.658^*$ & $0.657^*$ & $0.649^*$ & $0.731$ & $0.725$ & $0.685$ & $0.678$ \\
$\neg$ \centroidMacro & $0.639^*$ & $0.630^*$ & $0.630^*$ & $0.621^*$ & $0.676^*$ & $0.668^*$ & $0.694$ & $0.687$ \\
$\neg$ \docLen & $\mathbf{0.759}$ & $0.752$ & $0.741$ & $0.733$ & $\mathbf{0.796}$ & $\mathbf{0.792}$ & $0.713$ & $0.704$ \\
$\neg$ \PrevPosition & $0.713$ & $0.707$ & $0.722$ & $0.716$ & $0.750$ & $0.744$ & $0.694$ & $0.687$ \\
$\neg$ \QueryPrev & $\mathbf{0.759}$ & $\mathbf{0.753}$ & $\mathbf{0.787}$ & $\mathbf{0.780}$ & $0.657^*$ & $0.649^*$ & $\mathbf{0.750}$ & $\mathbf{0.743}$ \\
$\neg$ \PrevImprove & $0.741$ & $0.734$ & $0.769$ & $0.762$ & $0.769$ & $0.764$ & $0.731$ & $0.724$ \\
\allPredFeatures & $0.750$ & $0.742$ & $0.750$ & $0.742$ & $\mathbf{0.796}$ & $0.790$ & $\mathbf{0.750}$ & $\mathbf{0.743}$ \\
\bottomrule
\end{tabular}



==> tables/prediction/ablation_single.tex <==
\subcaption*{$LTR \wedge LLM$}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{LReg} & \multicolumn{2}{c}{LSVM} & \multicolumn{2}{c}{PSVM} & \multicolumn{2}{c}{RForest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
  &  &  &  &  &  &  &  &  \\
\midrule
\centroidMacro & 0.631 & 0.601 & 0.624 & 0.594 & 0.618 & 0.587 & 0.603 & 0.572 \\
\atomicFt & 0.686 & 0.67 & 0.686 & 0.669 & 0.717 & 0.699 & 0.663 & 0.641 \\
\metaFt & 0.717 & 0.701 & 0.717 & 0.701 & 0.714 & 0.694 & 0.735 & 0.719 \\
\PrevImprove & 0.594 & 0.553 & 0.604 & 0.564 & 0.575 & 0.538 & 0.504 & 0.459 \\
\QueryPrev & 0.544 & 0.505 & 0.541 & 0.502 & 0.529 & 0.489 & 0.531 & 0.493 \\
\docLen & 0.818 & 0.804 & 0.818 & 0.804 & 0.818 & 0.804 & 0.663 & 0.638 \\
\PrevPosition & 0.54 & 0.502 & 0.518 & 0.478 & 0.59 & 0.561 & 0.569 & 0.545 \\
\centroidMacro + \docLen + \metaFt + \atomicFt + \PrevPosition + \QueryPrev + \PrevImprove & \textbf{0.858} & \textbf{0.847} & \textbf{0.87} & \textbf{0.858} & \textbf{0.891} & \textbf{0.881} & \textbf{0.843} & \textbf{0.832} \\
\bottomrule
\end{tabular}

\bigskip
\subcaption*{$LTR \wedge \neg LLM$}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{LReg} & \multicolumn{2}{c}{LSVM} & \multicolumn{2}{c}{PSVM} & \multicolumn{2}{c}{RForest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
  &  &  &  &  &  &  &  &  \\
\midrule
\centroidMacro & 0.57 & 0.555 & 0.57 & 0.555 & 0.536 & 0.517 & 0.553 & 0.531 \\
\atomicFt & 0.66 & 0.645 & 0.666 & 0.651 & 0.667 & 0.656 & 0.727 & 0.718 \\
\metaFt & 0.728 & 0.715 & 0.728 & 0.715 & 0.711 & 0.697 & 0.769 & 0.758 \\
\PrevImprove & 0.549 & 0.523 & 0.555 & 0.53 & 0.524 & 0.498 & 0.576 & 0.558 \\
\QueryPrev & 0.57 & 0.551 & 0.57 & 0.551 & 0.623 & 0.607 & 0.591 & 0.574 \\
\docLen & 0.722 & 0.714 & 0.722 & 0.714 & 0.722 & 0.714 & 0.639 & 0.622 \\
\PrevPosition & 0.545 & 0.526 & 0.538 & 0.518 & 0.543 & 0.525 & 0.641 & 0.626 \\
\centroidMacro + \docLen + \metaFt + \atomicFt + \PrevPosition + \QueryPrev + \PrevImprove & \textbf{0.838} & \textbf{0.83} & \textbf{0.865} & \textbf{0.858} & \textbf{0.865} & \textbf{0.859} & \textbf{0.847} & \textbf{0.838} \\
\bottomrule
\end{tabular}

\bigskip
\subcaption*{$SEM \wedge LLM$}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{LReg} & \multicolumn{2}{c}{LSVM} & \multicolumn{2}{c}{PSVM} & \multicolumn{2}{c}{RForest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
  &  &  &  &  &  &  &  &  \\
\midrule
\centroidMacro & 0.608 & 0.579 & 0.615 & 0.587 & nan & nan & 0.545 & 0.51 \\
\atomicFt & 0.765 & 0.746 & 0.76 & 0.741 & 0.677 & 0.654 & 0.738 & 0.717 \\
\metaFt & 0.709 & 0.687 & 0.71 & 0.689 & 0.731 & 0.71 & 0.672 & 0.647 \\
\PrevImprove & 0.62 & 0.591 & 0.591 & 0.562 & 0.508 & 0.475 & 0.572 & 0.54 \\
\QueryPrev & 0.615 & 0.584 & 0.61 & 0.579 & 0.595 & 0.563 & 0.597 & 0.565 \\
\docLen & 0.559 & 0.523 & 0.565 & 0.529 & 0.521 & 0.483 & 0.488 & 0.447 \\
\PrevPosition & 0.503 & 0.471 & 0.503 & 0.471 & 0.525 & 0.492 & 0.565 & 0.534 \\
\centroidMacro + \docLen + \metaFt + \atomicFt + \PrevPosition + \QueryPrev + \PrevImprove & \textbf{0.811} & \textbf{0.797} & \textbf{0.803} & \textbf{0.788} & \textbf{0.814} & \textbf{0.798} & \textbf{0.826} & \textbf{0.812} \\
\bottomrule
\end{tabular}

\bigskip
\subcaption*{$SEM \wedge \neg LLM$}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{LReg} & \multicolumn{2}{c}{LSVM} & \multicolumn{2}{c}{PSVM} & \multicolumn{2}{c}{RForest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
  &  &  &  &  &  &  &  &  \\
\midrule
\centroidMacro & 0.457 & 0.446 & 0.435 & 0.424 & 0.443 & 0.432 & 0.555 & 0.545 \\
\atomicFt & 0.713 & 0.706 & 0.721 & 0.714 & 0.66 & 0.651 & 0.662 & 0.654 \\
\metaFt & 0.712 & 0.706 & 0.709 & 0.703 & 0.709 & 0.702 & 0.724 & 0.716 \\
\PrevImprove & 0.425 & 0.416 & 0.422 & 0.414 & 0.528 & 0.521 & 0.552 & 0.545 \\
\QueryPrev & 0.508 & 0.498 & 0.496 & 0.486 & 0.467 & 0.455 & 0.427 & 0.416 \\
\docLen & 0.395 & 0.382 & 0.393 & 0.38 & 0.421 & 0.408 & 0.513 & 0.5 \\
\PrevPosition & 0.479 & 0.469 & 0.469 & 0.459 & 0.525 & 0.515 & 0.461 & 0.45 \\
\centroidMacro + \docLen + \metaFt + \atomicFt + \PrevPosition + \QueryPrev + \PrevImprove & \textbf{0.781} & \textbf{0.774} & \textbf{0.784} & \textbf{0.778} & \textbf{0.785} & \textbf{0.779} & \textbf{0.752} & \textbf{0.746} \\
\bottomrule
\end{tabular}



==> tables/prediction/ablation_single_LReg.tex <==
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{\A} & \multicolumn{2}{c}{\B} & \multicolumn{2}{c}{\C} & \multicolumn{2}{c}{\D} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
\midrule
\atomicFt & $0.654^*$ & $0.635^*$ & $0.691^*$ & $0.678^*$ & $0.766$ & $0.747$ & $0.676$ & $0.670$ \\
\metaFt & $0.675^*$ & $0.656^*$ & $0.724^*$ & $0.711^*$ & $0.718^*$ & $0.695^*$ & $0.685$ & $0.679$ \\
\centroidMacro & $0.654^*$ & $0.623^*$ & $0.553^*$ & $0.533^*$ & $0.613^*$ & $0.581^*$ & $0.463^*$ & $0.454^*$ \\
\docLen & $\mathbf{0.822}$ & $0.809$ & $0.740^*$ & $0.731^*$ & $0.516^*$ & $0.476^*$ & $0.463^*$ & $0.451^*$ \\
\PrevPosition & $0.634^*$ & $0.606^*$ & $0.553^*$ & $0.536^*$ & $0.532^*$ & $0.497^*$ & $0.556^*$ & $0.546^*$ \\
\QueryPrev & $0.560^*$ & $0.521^*$ & $0.593^*$ & $0.576^*$ & $0.581^*$ & $0.546^*$ & $0.370^*$ & $0.361^*$ \\
\PrevImprove & $0.592^*$ & $0.555^*$ & $0.488^*$ & $0.461^*$ & $0.597^*$ & $0.564^*$ & $0.398^*$ & $0.388^*$ \\
\allPredFeatures & $\mathbf{0.822}$ & $\mathbf{0.810}$ & $\mathbf{0.886}$ & $\mathbf{0.879}$ & $\mathbf{0.815}$ & $\mathbf{0.800}$ & $\mathbf{0.750}$ & $\mathbf{0.742}$ \\
\bottomrule
\end{tabular}


==> tables/prediction/ablation_single_LSVM.tex <==
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{\A} & \multicolumn{2}{c}{\B} & \multicolumn{2}{c}{\C} & \multicolumn{2}{c}{\D} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
\midrule
\atomicFt & $0.623^*$ & $0.602^*$ & $0.699^*$ & $0.686^*$ & $0.758$ & $0.738$ & $0.694$ & $0.689$ \\
\metaFt & $0.675^*$ & $0.656^*$ & $0.724^*$ & $0.711^*$ & $0.718^*$ & $0.695^*$ & $0.685$ & $0.679$ \\
\centroidMacro & $0.654^*$ & $0.623^*$ & $0.553^*$ & $0.533^*$ & $0.613^*$ & $0.581^*$ & $0.407^*$ & $0.397^*$ \\
\docLen & $0.822$ & $0.809$ & $0.740^*$ & $0.731^*$ & $0.540^*$ & $0.502^*$ & $0.481^*$ & $0.470^*$ \\
\PrevPosition & $0.634^*$ & $0.606^*$ & $0.577^*$ & $0.560^*$ & $0.524^*$ & $0.488^*$ & $0.574^*$ & $0.565^*$ \\
\QueryPrev & $0.560^*$ & $0.521^*$ & $0.593^*$ & $0.576^*$ & $0.573^*$ & $0.537^*$ & $0.380^*$ & $0.370^*$ \\
\PrevImprove & $0.634^*$ & $0.600^*$ & $0.488^*$ & $0.461^*$ & $0.613^*$ & $0.580^*$ & $0.426^*$ & $0.416^*$ \\
\allPredFeatures & $\mathbf{0.853}$ & $\mathbf{0.843}$ & $\mathbf{0.870}$ & $\mathbf{0.863}$ & $\mathbf{0.798}$ & $\mathbf{0.782}$ & $\mathbf{0.750}$ & $\mathbf{0.742}$ \\
\bottomrule
\end{tabular}


==> tables/prediction/ablation_single_RForest.tex <==
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{\A} & \multicolumn{2}{c}{\B} & \multicolumn{2}{c}{\C} & \multicolumn{2}{c}{\D} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
\midrule
\atomicFt & $0.654^*$ & $0.633^*$ & $0.715^*$ & $0.704^*$ & $0.766^*$ & $0.746^*$ & $0.611^*$ & $0.605^*$ \\
\metaFt & $0.728^*$ & $0.712^*$ & $0.805$ & $0.799$ & $0.685^*$ & $0.660^*$ & $0.713$ & $0.705$ \\
\centroidMacro & $0.686^*$ & $0.660^*$ & $0.488^*$ & $0.463^*$ & $0.581^*$ & $0.546^*$ & $0.611^*$ & $0.603^*$ \\
\docLen & $0.728^*$ & $0.707^*$ & $0.715^*$ & $0.705^*$ & $0.444^*$ & $0.397^*$ & $0.519^*$ & $0.505^*$ \\
\PrevPosition & $0.728^*$ & $0.718^*$ & $0.634^*$ & $0.622^*$ & $0.524^*$ & $0.489^*$ & $0.565^*$ & $0.555^*$ \\
\QueryPrev & $0.560^*$ & $0.523^*$ & $0.610^*$ & $0.595^*$ & $0.589^*$ & $0.555^*$ & $0.463^*$ & $0.455^*$ \\
\PrevImprove & $0.602^*$ & $0.572^*$ & $0.528^*$ & $0.510^*$ & $0.645^*$ & $0.615^*$ & $0.565^*$ & $0.556^*$ \\
\allPredFeatures & $\mathbf{0.843}$ & $\mathbf{0.832}$ & $\mathbf{0.837}$ & $\mathbf{0.831}$ & $\mathbf{0.855}$ & $\mathbf{0.842}$ & $\mathbf{0.750}$ & $\mathbf{0.743}$ \\
\bottomrule
\end{tabular}


==> tables/prediction/ablation_single_all.tex <==
\subcaption*{\A}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{\lreg} & \multicolumn{2}{c}{\lsvm} & \multicolumn{2}{c}{\psvm} & \multicolumn{2}{c}{\rforest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
\midrule
\atomicFt & $0.654^*$ & $0.635^*$ & $0.623^*$ & $0.602^*$ & $0.613^*$ & $0.588^*$ & $0.654^*$ & $0.633^*$ \\
\metaFt & $0.675^*$ & $0.656^*$ & $0.675^*$ & $0.656^*$ & $0.665^*$ & $0.642^*$ & $0.728^*$ & $0.712^*$ \\
\centroidMacro & $0.654^*$ & $0.623^*$ & $0.654^*$ & $0.623^*$ & $0.696^*$ & $0.667^*$ & $0.686^*$ & $0.660^*$ \\
\docLen & $\mathbf{0.822}$ & $0.809$ & $0.822$ & $0.809$ & $0.822$ & $0.809$ & $0.728^*$ & $0.707^*$ \\
\PrevPosition & $0.634^*$ & $0.606^*$ & $0.634^*$ & $0.606^*$ & $0.581^*$ & $0.554^*$ & $0.728^*$ & $0.718^*$ \\
\QueryPrev & $0.560^*$ & $0.521^*$ & $0.560^*$ & $0.521^*$ & $0.550^*$ & $0.508^*$ & $0.560^*$ & $0.523^*$ \\
\PrevImprove & $0.592^*$ & $0.555^*$ & $0.634^*$ & $0.600^*$ & $0.560^*$ & $0.528^*$ & $0.602^*$ & $0.572^*$ \\
\allPredFeatures & $\mathbf{0.822}$ & $\mathbf{0.810}$ & $\mathbf{0.853}$ & $\mathbf{0.843}$ & $\mathbf{0.895}$ & $\mathbf{0.885}$ & $\mathbf{0.843}$ & $\mathbf{0.832}$ \\
\bottomrule
\end{tabular}

\bigskip
\subcaption*{\B}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{\lreg} & \multicolumn{2}{c}{\lsvm} & \multicolumn{2}{c}{\psvm} & \multicolumn{2}{c}{\rforest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
\midrule
\atomicFt & $0.691^*$ & $0.678^*$ & $0.699^*$ & $0.686^*$ & $0.634^*$ & $0.617^*$ & $0.715^*$ & $0.704^*$ \\
\metaFt & $0.724^*$ & $0.711^*$ & $0.724^*$ & $0.711^*$ & $0.667^*$ & $0.654^*$ & $0.805$ & $0.799$ \\
\centroidMacro & $0.553^*$ & $0.533^*$ & $0.553^*$ & $0.533^*$ & $0.577^*$ & $0.562^*$ & $0.488^*$ & $0.463^*$ \\
\docLen & $0.740^*$ & $0.731^*$ & $0.740^*$ & $0.731^*$ & $0.740^*$ & $0.731^*$ & $0.715^*$ & $0.705^*$ \\
\PrevPosition & $0.553^*$ & $0.536^*$ & $0.577^*$ & $0.560^*$ & $0.537^*$ & $0.515^*$ & $0.634^*$ & $0.622^*$ \\
\QueryPrev & $0.593^*$ & $0.576^*$ & $0.593^*$ & $0.576^*$ & $0.593^*$ & $0.580^*$ & $0.610^*$ & $0.595^*$ \\
\PrevImprove & $0.488^*$ & $0.461^*$ & $0.488^*$ & $0.461^*$ & $0.480^*$ & $0.452^*$ & $0.528^*$ & $0.510^*$ \\
\allPredFeatures & $\mathbf{0.886}$ & $\mathbf{0.879}$ & $\mathbf{0.870}$ & $\mathbf{0.863}$ & $\mathbf{0.846}$ & $\mathbf{0.839}$ & $\mathbf{0.837}$ & $\mathbf{0.831}$ \\
\bottomrule
\end{tabular}

\bigskip
\subcaption*{\C}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{\lreg} & \multicolumn{2}{c}{\lsvm} & \multicolumn{2}{c}{\psvm} & \multicolumn{2}{c}{\rforest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
\midrule
\atomicFt & $0.766$ & $0.747$ & $0.758$ & $0.738$ & $0.742$ & $0.720$ & $0.766^*$ & $0.746^*$ \\
\metaFt & $0.718^*$ & $0.695^*$ & $0.718^*$ & $0.695^*$ & $0.750$ & $0.729$ & $0.685^*$ & $0.660^*$ \\
\centroidMacro & $0.613^*$ & $0.581^*$ & $0.613^*$ & $0.581^*$ & $0.589^*$ & $0.554^*$ & $0.581^*$ & $0.546^*$ \\
\docLen & $0.516^*$ & $0.476^*$ & $0.540^*$ & $0.502^*$ & $0.468^*$ & $0.423^*$ & $0.444^*$ & $0.397^*$ \\
\PrevPosition & $0.532^*$ & $0.497^*$ & $0.524^*$ & $0.488^*$ & $0.524^*$ & $0.489^*$ & $0.524^*$ & $0.489^*$ \\
\QueryPrev & $0.581^*$ & $0.546^*$ & $0.573^*$ & $0.537^*$ & $0.500^*$ & $0.458^*$ & $0.589^*$ & $0.555^*$ \\
\PrevImprove & $0.597^*$ & $0.564^*$ & $0.613^*$ & $0.580^*$ & $0.556^*$ & $0.521^*$ & $0.645^*$ & $0.615^*$ \\
\allPredFeatures & $\mathbf{0.815}$ & $\mathbf{0.800}$ & $\mathbf{0.798}$ & $\mathbf{0.782}$ & $\mathbf{0.806}$ & $\mathbf{0.790}$ & $\mathbf{0.855}$ & $\mathbf{0.842}$ \\
\bottomrule
\end{tabular}

\bigskip
\subcaption*{\D}
\begin{tabular}{lllllllll}
\toprule
  & \multicolumn{2}{c}{\lreg} & \multicolumn{2}{c}{\lsvm} & \multicolumn{2}{c}{\psvm} & \multicolumn{2}{c}{\rforest} \\
  & \acc & \FOne & \acc & \FOne & \acc & \FOne & \acc & \FOne \\
\midrule
\atomicFt & $0.676$ & $0.670$ & $0.694$ & $0.689$ & $0.602^*$ & $0.593^*$ & $0.611^*$ & $0.605^*$ \\
\metaFt & $0.685$ & $0.679$ & $0.685$ & $0.679$ & $0.639^*$ & $0.633^*$ & $0.713$ & $0.705$ \\
\centroidMacro & $0.463^*$ & $0.454^*$ & $0.407^*$ & $0.397^*$ & $0.463^*$ & $0.455^*$ & $0.611^*$ & $0.603^*$ \\
\docLen & $0.463^*$ & $0.451^*$ & $0.481^*$ & $0.470^*$ & $0.556^*$ & $0.551^*$ & $0.519^*$ & $0.505^*$ \\
\PrevPosition & $0.556^*$ & $0.546^*$ & $0.574^*$ & $0.565^*$ & $0.583^*$ & $0.575^*$ & $0.565^*$ & $0.555^*$ \\
\QueryPrev & $0.370^*$ & $0.361^*$ & $0.380^*$ & $0.370^*$ & $0.509^*$ & $0.502^*$ & $0.463^*$ & $0.455^*$ \\
\PrevImprove & $0.398^*$ & $0.388^*$ & $0.426^*$ & $0.416^*$ & $0.519^*$ & $0.509^*$ & $0.565^*$ & $0.556^*$ \\
\allPredFeatures & $\mathbf{0.750}$ & $\mathbf{0.742}$ & $\mathbf{0.750}$ & $\mathbf{0.742}$ & $\mathbf{0.796}$ & $\mathbf{0.790}$ & $\mathbf{0.750}$ & $\mathbf{0.743}$ \\
\bottomrule
\end{tabular}



==> tables/prediction/table12.tex <==
\begin{tabular}{llllllllllll}
\toprule
group & metric & Random & Query Majority & Topic Majority & All Winners & All Losers & RForest(Micro+Macro) & LReg(All) & PSVM(All) & LSVM(All) & RForest(All) \\
\midrule
$LTR \wedge LLM$ & accuracy & 0.623 & 0.435 & 0.503 & 0.466 & 0.534 & 0.757 & 0.858 & 0.87 & \textbf{0.891} & 0.843 \\
$LTR \wedge LLM$ & f1 & 0.591 & 0.397 & 0.497 & 0.635 & 0.0 & 0.743 & 0.847 & 0.858 & \textbf{0.881} & 0.832 \\
$LTR \wedge \neg LLM$ & accuracy & 0.707 & 0.398 & 0.504 & 0.48 & 0.52 & 0.791 & 0.838 & \textbf{0.865} & \textbf{0.865} & 0.847 \\
$LTR \wedge \neg LLM$ & f1 & 0.697 & 0.368 & 0.497 & 0.648 & 0.0 & 0.783 & 0.83 & 0.858 & \textbf{0.859} & 0.838 \\
$SEM \wedge LLM$ & accuracy & 0.677 & 0.532 & 0.468 & 0.464 & 0.536 & 0.713 & 0.811 & 0.803 & 0.814 & \textbf{0.826} \\
$SEM \wedge LLM$ & f1 & 0.651 & 0.495 & 0.588 & 0.634 & 0.0 & 0.692 & 0.797 & 0.788 & 0.798 & \textbf{0.812} \\
$SEM \wedge \neg LLM$ & accuracy & 0.639 & 0.481 & 0.5 & 0.491 & 0.509 & 0.72 & 0.781 & 0.784 & \textbf{0.785} & 0.752 \\
$SEM \wedge \neg LLM$ & f1 & 0.631 & 0.471 & 0.592 & 0.658 & 0.0 & 0.712 & 0.774 & 0.778 & \textbf{0.779} & 0.746 \\
\bottomrule
\end{tabular}


==> tables/prediction/table13.tex <==
\begin{tabular}{@{}llllllllllll@{}}
\toprule
  &   & \random & \qmajority & \tmajority & \awinner & \aloser & \nimrodBest & \lreg & \lsvm & \psvm & \rforest \\
\midrule
\A & \acc & 0.654 & 0.435 & 0.503 & 0.466 & 0.534 & 0.696 & 0.822 & 0.853 & \textbf{0.895} & 0.843 \\
\A & \FOne & 0.622 & 0.397 & 0.497 & 0.635 & 0.000 & 0.678 & 0.810 & 0.843 & \textbf{0.885} & 0.832 \\ \midrule
\B & \acc & 0.707 & 0.398 & 0.504 & 0.480 & 0.520 & 0.772 & \textbf{0.886} & 0.870 & 0.846 & 0.837 \\
\B & \FOne & 0.697 & 0.368 & 0.497 & 0.648 & 0.000 & 0.763 & \textbf{0.879} & 0.863 & 0.839 & 0.831 \\ \midrule
\C & \acc & 0.669 & 0.532 & 0.468 & 0.464 & 0.536 & 0.766 & 0.815 & 0.798 & 0.806 & \textbf{0.855} \\
\C & \FOne & 0.643 & 0.495 & 0.588 & 0.634 & 0.000 & 0.747 & 0.800 & 0.782 & 0.790 & \textbf{0.842} \\ \midrule
\D & \acc & 0.556 & 0.481 & 0.500 & 0.491 & 0.509 & 0.722 & 0.750 & 0.750 & \textbf{0.796} & 0.750 \\
\D & \FOne & 0.547 & 0.471 & 0.592 & 0.658 & 0.000 & 0.717 & 0.742 & 0.742 & \textbf{0.790} & 0.743 \\
\bottomrule
\end{tabular}
